MelBERT: Metaphor Detection via Contextualized Late Interaction using Metaphorical Identification Theories

Automated metaphor detection is a challenging task to identify metaphorical expressions of words in a sentence. To tackle this problem, we adopt pre-trained contextualized models, e.g., BERT and RoBERTa. To this end, we propose a novel metaphor detection model, namely metaphor-aware late interaction over BERT (MelBERT). Our model not only leverages contextualized word representation but also benefits from linguistic metaphor identification theories to distinguish between the contextual and literal meaning of words. Our empirical results demonstrate that MelBERT outperforms several strong baselines on four benchmark datasets, i.e., VUA-18, VUA-20, MOH-X, and TroFi.

==> Backup/sec-background.tex <==
\section{Background}

For the metaphor detection problem, we can consider two linguistic metaphor theories. In \emph{selectional preference violence} (\emph{SPV})~\cite{Wilks75, Wilks78}, a metaphorical word is identified by the semantic difference from its surrounding words.
In \emph{metaphor identification procedure} (\emph{MIP})~\cite{Group2007mip},  a metaphor is regarded by the gap between contextual and literal meaning of it. As BERT inherently considers the surrounding words of a given word, we focus on MIP. 


Although the literal and metaphoric words are provided by datasets, we explain literal and metaphor meaning of a word. The ``literal'' meaning of a word is the historically oldest and common meanings of a given word. Meanwhile, the ``metaphoric'' meaning of a word is relatively new, rare meanings of a given word. The ``metaphoric'' word can also be understand by surrounding contexts. Besides, the metaphorical ``novelty'' is measured by the gap from the literal meaning. 



%This way might not be logical but determinate~\cite{stockwell2001english}. 
%Based on this idea, Many dictionaries (\eg, \cite{staff2004merriam}) and MIP adopt it to arrange words' senses.
% ``metaphor''
% ``metaphor''
% To determine what is metaphor, in this paper, we assumed the first dictionary meaning of each word as the literal meaning of the word and all the other meanings as metaphoric meanings.

==> Backup/sec-conclusion.tex <==
\section{Conclusion}

In this paper, we proposed \emph{BERT with Linguistic metaphor Theories (BLT)} for detecting metaphors. To our best knowledge, this is the first work that takes full advantage of BERT using a linguistic metaphor theory, MIP. Our empirical study revealed that our models achieve state-of-the-art performance on several benchmark datasets. 

==> Backup/sec-experiments.tex <==
\input{Tables/tab-dataset}
\input{Tables/tab-main}


\section{Experiments}

%In this section, we first explain the experimental setup, then report the experimental results by comparing our models against baselines.


\subsection{Experimental Setup}


\noindent
\textbf{Dataset}. We used four well-known public datasets, three for metaphor detection and one for novelty regression: \emph{(i)} the VU Amsterdam Metaphor Corpus (VUA)~\cite{Steen2010method}, consisting of VUA\_ALL for sequence labeling and VUA\_VERB for verb classification, \emph{(ii)} MOH-X~\cite{MohammadST16} for classification, built from WordNet~\cite{Miller1998wordnet}, \emph{(iii)} TroFi~\cite{BirkeS06} for classification, built from 1987-89 Wall Street Journal Corpus Release 1~\cite{Charniak2000bllip}, \emph{(iv)} LCC~\cite{mohler2016introducing}, collected from ClueWeb09\footnote{\url{http://lemurproject.org/clueweb09/}}. Detailed dataset statistics are summarized in Table~\ref{tab:dataset}.


\vspace{1mm}
\noindent
\textbf{Baselines}. We compared our models with three baselines: (i) \emph{RNN\_ELMo, RNN\_BERT}~\cite{GaoCCZ18} input the concatenation of the pre-trained ELMo/BERT layers and the GloVe~\cite{PenningtonSM14} embeddings into the BiLSTM, then classify every word in a sentence. 
(ii) \emph{RNN\_HG, RNN\_MHCA}~\cite{MaoLG19} apply MIP and SPV to \emph{RNN\_ELMo}, respectively. \emph{RNN\_HG} compares the input embedding (literal) with the hidden state (contextual). \emph{RNN\_MHCA} utilizes multi-head attention to capture the context feature within the window.
(iii) \emph{CLS\_BASE, SEQ\_BASE}: For ablation study, we designed the variant of BLT\_CLS and BLT\_SEQ, without the isolated target word and the concatenation step, respectively.

\vspace{1mm}
\noindent
\textbf{Evaluation}. For MOH-X, TroFi, and LCC, few words in a sentence are labeled. When training BLT\_SEQ, we assume that all words but a target are literal. We conduct 10-fold cross-validation for MOH-X and TroFi. For VUA, we only use VUA\_ALL for training BLT\_SEQ and employ both VUA\_ALL and VUA\_VERB for evaluation.
% As to metrics, we use precision, recall, and F1 for classification and Spearman/Pearson correlation for regression.

\vspace{1mm}
\noindent
\textbf{Implementation details}. For four baselines, we use the same parameter settings in~\cite{GaoCCZ18, MaoLG19}. For our model, we set batch size and max sequence length as 32 and 200, respectively. We increase the learning rate from 0 to 5e-5 during the first half of the training with Adam optimizer, and then linearly decrease it during the second half. We use a pre-trained BERT-base with 12 layers, 12 attention heads in each layer, and 768 dimensions of the hidden state. To adjust the imbalanced labels in datasets, we use the weighted cross-entropy loss, with 10 times weights to metaphors for all datasets in BLT\_SEQ and 3 times for VUA and no weight for the others in BLT\_CLS.

%\footnote{\href{https://storage.googleapis.com/bert_models/2018_10_18/cased_L-12_H-768_A-12.zip}{https://storage.googleapis.com/bert\_models/2018\_10\_18/cased\_L-12\_H-768\_A-12.zip}}


\subsection{Experimental Results}

\noindent
\textbf{Overall results}. Table~\ref{tab:overall} shows that BLT performs consistently better than or comparable to the competing models, with the following observations:

\noindent
$\bullet$ Effectiveness of our models: BLT\_SEQ achieves the state-of-the-art performance on VUA\_ALL and VUA\_VERB, with 2.3\% and 3.9\% performance gains comparing to RNN\_MHCA. For MOH-X, both BLT\_CLS and BLT\_SEQ (F1 = 82.3\%, 81.4\%) outperform RNN\_MHCA (F1 = 80.0\%). For TroFi, BLT\_CLS is comparable to RNN\_MHCA with a small difference (0.1\%).

\noindent
$\bullet$ Effectiveness of BERT scheme: Compared with RNN\_BERT, BLT shows about 2--5\% performance gains in F1 on all datasets, indicating that utilizing BERT as a backbone model has a better effect than simply utilizing it as extra embeddings.

\noindent
$\bullet$ Effectiveness of MIP theory: Compared with CLS/SEQ\_BASE, our models achieve up to 3\% performance gains in F1-measure. That is, incorporating MIP into BERT can be more effective than using BERT only.

\noindent
$\bullet$ Trade-off between metrics: While sequential labeling models are worse than classification models in terms of precision, sequential labeling shows better than classification in terms of recall. We conjecture that the trade-off between precision and recall comes from the sparsity of labels. That is, sequential labeling considers all words, but the classification only checks a target word. 


%\noindent
%$\bullet$ Difficulty in training sequential labeling models: 


%MOH-X and TroFi datasets. Because MOH-X mainly consists of short sentences, it is more favorable to classification. For TroF
%Notably, because the TroFi dataset consists of longer sequences with some non-labeled metaphors, we assume that all words are literal except for a target word, which makes it difficult to apply for sequential labeling.

%The results on MOH-X and TroFi show that BLT\_CLS performs better than BLT\_SEQ with sparse labels. While MOH-X consists of short sequences with a clear context, Trofi consists of much, contrary to our assumption for BLT\_SEQ that all words but a target are literal.
% As shown in Table~\ref{tab:overall}, our models perform consistently better than or comparable to the competing models. BLT\_SEQ achieves state-of-the-art performance on VUA\_ALL and VUA\_VERB (F1 = 76.6\%, 74.3\%). Compared to RNN\_MHCA, its performance gains are 2.3\% and 3.9\%, respectively. For MOH-X, both BLT\_CLS and BLT\_SEQ (F1 = 82.3\%, 81.4\%) outperform RNN\_MHCA (F1 = 80.0\%). For TroFi, BLT\_CLS is comparable to RNN\_MHCA with a small difference (0.1\%). 


\input{Tables/tab-genre}

\vspace{1mm}
\noindent
\textbf{VUA breakdown analysis}. Table~\ref{tab:breakdown} reports the performances in four genres in VUA\_ALL. Our models significantly outperform all competitive models. Compared to RNN\_MHCA, BLT\_SEQ achieves substantial improvements, as high as 4.2\% (Academic) and 5.7\% (Fiction). In particular, we found that Fiction includes more complicated or rare expressions than other types. For example, in ``Oh! She squealed as \emph{light dawned}'', the phrase ``\emph{light dawned}'' is regarded as a metaphor. For the rare use, while existing models cannot detect it, our models can identify such rare metaphorical expressions. For POS tags, our models consistently show significant gains, as much as 4.1\% (Verb), 3.3\% (Adjective), 6.2\% (Adverb), and 5.5\% (Noun)\footnote{Due to the page limitation, we omit this result.}.


\vspace{1mm}
\noindent
\textbf{Ablation study of MelBERT}.

\input{Tables/tab_error}

\vspace{1mm}
\noindent
\textbf{Error analysis}. As shown in Table~\ref{tab:errorcase}, we report several interesting observations: (i) BLT\_CLS often fails to detect metaphorical words with different meanings or roles. For instance, ``hit'' has multiple meanings such as ``to strike'' and ``base hit in a baseball game.'' Similarly, ``damage'' is used as either a noun or a verb. (ii) BLT\_SEQ is difficult to distinguish literal words near metaphorical words, \eg, BLT\_SEQ incorrectly regards ``neck'' and ``inside'' as metaphors near metaphorical words ``chicken'' and ``bubbling,'' respectively. (iii) Due to the lack of context, both models struggle in identifying metaphors for too short sentences.

\input{Tables/tab-regression}

\vspace{1mm}
\noindent
\textbf{Metaphor novelty regression}. To explore the potential of our model, we extend our model for metaphor novelty regression by simply adopting mean squared error as a loss function. In Table~\ref{tab:regression}, the predictions of our models show a high correlation (over 0.7 in Spearman's $\rho$ and Pearson's $r$) with ground truth. BLT\_CLS still outperforms BLT\_SEQ in LCC dataset. Also, compared with CLS\_BASE, the effect of MIP to BLT\_CLS is also meaningful for the regression task.

==> Backup/sec-introduction.tex <==
\section{Introduction}

The goal of automated metaphor detection is to identify figurative and unusual words that enrich the linguistic expressions of humans~\cite{Wilks75, Lakoff2008metaphors} using computational NLP models. For instance, in the sentence ``the ballerina was a swan,'' the word ``swan'' does not literally mean a white bird living on a lake. Instead, it is a metaphorical expression to describe the graceful movement of the ballerina. The meaning of ``swan'' is, therefore, context-specific and different from its conventional word definition. As metaphorical expressions commonly appear in various NLP applications (\eg, machine translation~\cite{Shi2014translation}, sentimental analysis~\cite{Cambria2017sentiment}, and dialog systems~\cite{Dybala2013metaphor}, it is critical for machines to be capable of correctly understanding the semantic meanings of words.



Existing studies for metaphor detection can be categorized into two camps. The conventional approaches detect the metaphors in phrase-level or word pairs under limited linguistic contexts~\cite{TurneyNAC11,BroadwellBCSFTSLCW13,ShutovaKM16,ReiBKS17}. On the other hand, recent approaches generalize the metaphor detection problem by utilizing pre-trained word embeddings~\cite{MaoLG18}, \eg, word2vec~\cite{MikolovSCCD13}, or adopting the RNN-based model~\cite{WuWCWYH18, GaoCCZ18, MaoLG19} to learn the contextualized features of words. However, recent a few studies take advantage of pre-trained language models, which are known to better capture contextual features of words.


\input{Figures/fig-MelBERT-MIP}
\input{Figures/fig-MelBERT-SPV}

In this paper, we utilize a well-known representative pre-trained language model, \ie, BERT~\cite{DevlinCLT19}. Owing to the powerful contextualized representation of words, BERT has been successfully used as a backbone model to address various natural language understanding (NLU) tasks, \eg,~\cite{wang2018glue,zellers2018swag}. Although some recent studies attempt to use ELMo or BERT for detecting metaphors, they simply utilize it as pre-defined word embedding~\cite{GaoCCZ18, MaoLG19}. In contrast, we incorporate BERT into metaphor identification theories. We make use of \emph{metaphor identification procedure (MIP)}~\cite{Group2007mip} and \emph{selectional preference violence (SPV)}~\cite{Wilks75, Wilks78} to distinguish between the contextualized meaning and the conventional definition of a target word. 


To this end, we propose a novel metaphor detection model, namely \emph{metaphor-aware late interaction over BERT} (\emph{MelBERT}). The proposed model deals with a classification task to identify whether a target word in a sentence is metaphorical or not. Given a sentence, MelBERT first utilizes siamese BERT that takes two sentences, where one sentence only is represented by a target word, to distinguish between the contextualized meaning and the literal meaning of the target word using MIP (Figure~\ref{fig:melbert-mip}). Also, MelBERT considers the [CLS] token to distinguish the semantic gap between the sentence representation and the word token representation using SPV (Figure~\ref{fig:melbert-spv}). Lastly, MelBERT synergizes to predict metaphors by combining two components. Experimental results show that MelBERT outperforms state-of-the-art methods by up to XX--XX\% in several benchmark datasets, such as VUA\_ALL, VUA\_VERB, TOEFL, MOH-X, and TroFi.





%\vspace{1mm}


==> Backup/sec-model.tex <==
\section{MelBERT: Proposed Models}

Although the ground-truth for literal or metaphorical words is provided by benchmark datasets, we clarify the literal and metaphoric meanings of a word. The ``literal'' meaning of a word is historically oldest or ordinary~\cite{stockwell2001english,staff2004merriam}. Meanwhile, the ``metaphoric'' meaning of a word is relatively new or rare. 


For the classification task, it takes a sentence including a target word as input and returns a binary output, \ie, 1 if the target word is metaphorical and 0 otherwise. In this process, we develop a novel metaphor detection model, namely, \emph{metaphor-aware late interaction over BERT} (\emph{MelBERT}), which metaphor identification theories incorporates into BERT. In \emph{metaphor identification procedure} (\emph{MIP})~\cite{Group2007mip},  a metaphor is identified by the gap between contextual and literal meaning of it. In \emph{selectional preference violence} (\emph{SPV})~\cite{Wilks75, Wilks78}, a metaphorical word is identified by the semantic difference from its surrounding words. Because BERT is capable of capturing contextualized meanings of an entire sentence and the words in the sentence, we can utilize them to distinguish a semantic gap of sentence and words.




Figure~\ref{fig:mlb-cls} illustrates the first component of MelBERT using MIP. Specifically, we utilize siamese BERT to distinguish between the context-specific meaning and the literal meaning of a target word. One input sentence including a target word is taken as input, where BERT can capture the contextualized meaning of the target word in the sentence. Another input sentence is represented by an isolated target word to capture a literal meaning of the target word. Then, we can distinguish the semantic gap between the original target word in contexts and the isolated target word. That is, we feedback two hidden states $h_c$ and $h_l$ of target word token to a softmax layer $\sigma$ after linearly transforming it with learned parameters $w$ and $b$:
\begin{equation}
p(\hat{y}_t | s, c) = \sigma(w^{\top} [h_c; h_l] + b),
\end{equation}
\noindent
where $s$ and $c$ indicate the sentence and the isolated target word.



%We then add direction embeddings to the target word (T in Figure~\ref{fig:mlb-cls}) in contexts and the isolated one (W in Figure~\ref{fig:mlb-cls}) 

Figure~\ref{fig:mlb-seq} depicts the second component of MelBERT using SPV. Unlike the first component, it simply takes a sentence as input. To distinguish the semantic gap between the sentence and a target word, it utilizes [CLS] token and the target word token. While the first embedding vector represents the sentence representation including the surrounding words of the target word, the second embedding vector represents the word representation for the target word. Therefore, it can learn the semantic gap between two vectors. For a target word at $t$-th position, the likelihood is calculated as follows.
\begin{equation}
p(\hat{y}_t | s, c) = \sigma(w'^{\top} [h_[CLS]; h_t] + b').
\end{equation}


Lastly, we combine two components.

%\noindent
%where $e_t$ and $h_t$ denote the input and the output vector of BERT for a target word.

%For the metaphor detection problem, we can consider two linguistic metaphor theories. In \emph{selectional preference violence} (\emph{SPV})~\cite{Wilks75, Wilks78}, a metaphorical word is identified by the semantic difference from its surrounding words. In \emph{metaphor identification procedure} (\emph{MIP})~\cite{Group2007mip},  a metaphor is identified by the gap between contextual and literal meaning of it.
%In addition, the metaphorical ``novelty'' is measured by the semantic gap between the literal and the metaphoric meaning of a word.


==> Tables/tab-ablation_token.tex <==
\begin{table}[t]
\begin{small}
\begin{center}
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{VUA-18}                    & \multicolumn{3}{c}{VUA-20}                   \\
                       & F1            & Prec          & Rec           & F1            & Prec          & Rec           \\ \midrule
MelBERT                & 78.5          & 80.1          & 76.9          & 72.3          & {\ul 76.4}    & 68.6          \\
(-) POS                & {\ul 78.6}    & {\ul 80.4}    & {\ul 76.9}    & 72.0          & 74.7          & 68.0          \\
(-) Local              & \textbf{78.8} & 80.1          & \textbf{77.6} & {\ul 72.4}    & 75.7          & \textbf{69.4} \\
No features         & 78.6          & \textbf{80.8} & 76.6          & \textbf{72.6} & \textbf{76.9} & {\ul 68.7}    \\ \bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{-2mm}
\caption{Effect of different linguistic features over MelBERT on VUA-18 and VUA-20. Let (-) Local and (-) POS denote MelBERT without local context and POS tag features, respectively.}\label{tab:ablation_token}
\end{table}



% \toprule
% \multirow{2}{*}{Model} & \multicolumn{3}{c}{VUA-18}                  & \multicolumn{3}{c}{VUA-20}                 \\
%                       & F1            & P             & R             & F1            & P             & R             \\ \midrule
% MelBERT                & 71.5          & 76.6          & 67.0          & \textbf{76.0} & 79.1          & \textbf{73.2} \\
% (-) Local              & 71.4          & 75.9          & 67.4          & 74.6          & 77.8          & 71.6          \\
% (-) POS \ \                & 72.0          & 67.5          & 67.5          & 75.3          & 79.3          & 71.6          \\
% No features         & \textbf{72.4} & \textbf{77.8} & \textbf{67.7} & 75.6          & \textbf{80.2} & 71.4          \\ \bottomrule
